Improving Bilingual Capabilities of Language Models to Support Diverse Linguistic Practices in Education

Large language models (LLMs) offer promise in generating educational content, providing instructor feedback, and reducing teacher workload on assessments. While prior studies have focused on studying LLM-powered learning analytics, limited research has examined how effective LLMs are in a bilingual context. In this paper, we study the effectiveness of multilingual large language models (MLLMs) across monolingual (English-only, Spanish-only) and bilingual (Spanglish) student writing. We present a learning analytics use case that details LLM performance in assessing acceptable and unacceptable explanations of Science and Social Science concepts. Our findings reveal a significant bias in the grading performance of pre-trained models for bilingual writing compared to English-only and Spanish-only writing. Following this, we fine-tune open-source MLLMs including Llama 3.1 and Mistral NeMo using synthetic datasets generated in English, Spanish, and Spanglish. Our experiments indicate that the models perform significantly better for all three languages after fine-tuning with bilingual data. This study highlights the potential of enhancing MLLM effectiveness to support authentic language practices amongst bilingual learners. It also aims to illustrate the value of incorporating non-English languages into the design and implementation of language models in education.

==> Sections/02_related_work.tex <==
% \section{Related Work}
% In this paper, we seek to investigate the translanguaging abilities of Multilingual Large Language Models (MLLMs) in the context of education. Building upon existing research on translanguaging, bilingualism, and the current NLP techniques, this research necessitates the integration of emergent bilingual learners' experiences and accompanying linguistic backgrounds into the training and processing of MLLMs.
% \label{sec:related-work}

% \subsection{Translanguaging}


% The phenomenon of translanguaging provides a theoretical lens to the pedagogical and fluid language practices of bilingual and multilingual learners (Wei, L. 2018; García, O., \& Lin, A. M. 2017). Within this framework, speakers draw from their entire linguistic background rather than conform to socio-political boundaries of named languages (Otheguy, Garcia \& Reid, 2015), oftentimes guided by communicative intent with interlocutors. In this section, we discuss the goals and applications of translanguaging as both a theoretical framework and pedagogical practice, as well as current issues surrounding bilingual education practices and ideologies.

% \subsubsection{Translanguaging, Code-Switching and Bilingualism}

% While scholarly literature provides contrasting perspectives on the current use of translanguaging, it is clear that its value lies in the intersectionality of language and social justice. For instance, Li Wei (2011) defines the term translanguaging space as a place where cultural and linguistic boundaries are eclipsed in bi-/multilinguals’ daily lives. Within these spaces, both criticality and creativity work simultaneously to inform perceptions on socio-cultural and linguistic phenomena and determine what constitutes the norms of language use. Translanguaging, therefore, extends beyond the many pre-existing multilingual frameworks that have sought to categorize ‘proper’ language use, including code-switching, code-mixing, code-meshing, crossing, etc.

% As a communicative form, code-switching is described as 1.) the alternating use between two distinct named languages (i.e., Spanish and English) following consistent grammatical rules and 2.) the integration of these languages as characterized by word borrowings and lexical adaptation (Price, 2010). Take, for example, an emergent bilingual learner (EBL) using Spanglish to explain a scientific phenomenon in a classroom. By code-switching, this learner may go back and forth between languages to explain a particular scientific concept or idea. Under this assumption, however, less value is given to the multifaceted linguistic and semiotic resources, including the space itself, from which the EBL draws from in order to get there. In other words, code-switching only constitutes one aspect of translanguaging. García \& Lin (2017) argue that this is accentuated by the fact that code-switching, when done pragmatically, aims to incorporate multiple languages in isolation rather than sustain bilingualism altogether. We therefore use translanguaging as an epistemological stance to describe the fuller picture of an emergent bilingual’s linguistic background and decisions regardless of the artificial divides between named languages.	


% \subsubsection{Bilingualism and Translanguaging in Education}

% Much research has been done in U.S. education systems to identify areas of support for emergent bilingual learners. Despite this, the understanding that English remains the lingua franca and takes priority in most U.S. schools is still as prevalent as it was decades ago. García (2020) states that even in English-Spanish classrooms, Latinx bilinguals have less access to their linguistic background when being assessed on literacy, most likely due to teachers having a monoglossic view on the linguistic features deemed valid in school texts. Equally concerning, dual-language programs, which seek to develop students’ proficiency in two or more languages, often maintain language separation to produce monolingual speakers of different languages (Palmer et al., 2014). Major developments in bilingual education aim to reframe these ideologies. By de-centering the idea that learning English is the cornerstone of success, there is an inherent need for translanguaging practices to be recognized at scale to maintain the full acceptance of emergent bilingual learners.
% To further understand the scope of translanguaging, we must also address its overarching goal within educational contexts. Translanguaging fosters equitable learning outcomes by encouraging fluid language use, in turn promoting authentic social interaction and communication within the classroom (Hamman, 2017). This is achieved by utilizing students’ existing language background, cultural identity, and multimodal practices (i.e., gesture) as meaning-making processes. Translanguaging pedagogy also promotes linguistic appropriate practices (Cummins, 2019), whereby EBLs acknowledge their unique linguistic system and literacy needs by charting and integrating their home language(s) and cultural practices into the classroom, in turn promoting bilingualism and family partnerships. Additionally, students’ who saw the benefits of translanguaging directly related its acceptance to their own language learning and vocabulary development (Öztürk \& Çubukçu, 2022). These practices, guided by the allowance of translanguaging ideology and practice, help to promote inclusivity and bridge the gap between students’ personal and academic worlds.

% \subsubsection{Local and Global Perspectives on Translanguaging in K-12 Classrooms} Much of translanguaging discourse has shifted towards how to leverage students’ primary linguistic resources in learning environments. Within the U.S., curricula and instructional resources now include pedagogical strategies that use bilingualism as a resource to leverage learning. In response to the Common Core's pervasive influence across the country, the CUNY-NYSIEB Guide for Educators was created to enable EBLs to meet these rigorous standards. Today, six CUNY-NYSIEB guides exist that detail the ways educators can bring translanguaging into the classroom, from emphasizing collaborative work and multilingual resources to building upon multilingual vocabulary and sentence structure (Hessen, Seltzer \& Woodley, 2014). They also provide tailored strategies for varying age and grade levels, from elementary to high school. This growing body of resources has been widely used by educational communities working towards putting theory into practice.	

% With increasing globalization, current translanguaging practices are also being promoted at an international scale to challenge traditional notions of bilingualism in education. For instance, scholars and  researchers alike have collaborated to draw from local experiences in order to advocate for more inclusive multilingual educational frameworks and promote fluid language use in education globally (Skutnabb-Kangas et al., 2009). This is in part a response to English linguistic hegemony that has revealed itself in both the U.S. and EU systems through exclusion of minority languages from local and global school systems, the de facto hierarchy of languages, and inequality between native English speakers and other Europeans in international communication (Phillipson, 2009). As research in this field advances in both the U.S. and globally, we view translanguaging as an increasingly valuable pedagogical approach that empowers EBLs to communicate by leveraging their diverse linguistic and meaning-making resources.

% \subsection{LLM Support for Student Learning}

% \subsubsection{LLMs}

% Large Language Models (LLMs), such as GPT-4, have become prominent in natural language processing (NLP). They are able to understand and generate human language through being pretrained on language datasets at large sizes (Vaswani et al., 2017; Brown et al., 2020). In tasks in educational settings like essay scoring and feedback generation, they are potential to tackle challenges that traditional methods struggled with.

% \subsubsection{NLP in Education}
% Automated Essay Scoring (AES) systems have been pivotal in enabling large-scale assessments by allowing learners to practice writing independently while reducing examiner workloads (Nguyen et al., 2022). They have been widely used in standardized tests like TOEFL and GMAT (Chen et al., 2016; Chodorow \& Burstein, 2004) and in classrooms (Wilson et al., 2019). Early systems like IntelliMetric (Elliot, 2003) and E-rater® (Attali \& Burstein, 2006) relied on manually engineered features like essay length, making them vulnerable to manipulation and less effective in assessing essay quality (Fazal et al., 2011; Davis, 2014; Greene, 2018). Later approaches addressed these issues by incorporating deep learning techniques, including CNNs, LSTMs, and transformers (Taghipour \& Ng, 2016; Alikaniotis et al., 2016; Liang et al., 2018). Transformer models like BERT are now setting the benchmark for AES (Hirao et al., 2020; Andersen et al., 2021; Wang et al., 2022; Boquio \& Naval, 2024), among which LLMs are now viewed as the most promising tools (Song et al., 2024; Li \& Liu, 2024; Andersen et al., 2021).

% Besides scoring, researchers are looking to intelligent tutoring systems and computer-based to provide high-quality, personalized, and timely feedback, which can significantly improve learner outcomes (Hattie \& Timperley, 2007). However, generating such feedback remains a challenge (Maniktala et al., 2020). Early feedback generation methods had limited flexibility since they relied on template-based methods (Liu et al., 2016; Blayney \& Freeman, 2004). Though most previous studies have been able to provide sentence-level feedback (Zupanc \& Bosnić, 2017; Woods et al., 2017), holistic, essay-level feedback remains underexplored. The lack of annotated datasets poses another significant challenge, leading some researchers to develop their own corpora (Ke et al., 2020). LLMs demonstrate significant potential in addressing these challenges (Stahl et al., 2024; Meyer et al., 2024).

% \subsubsection{Early Explorations of LLMs in Classroom Settings}

% LLMs have also shown potential in specific subjects. In mathematics, for example, LLMs have been used to generate multiple-choice questions (Nichols et al., 2024), select math problems for tutoring (Levonian et al., 2023), plot math figures (Bulusu et al., 2023), collaborate with teachers to collect tutoring data and fine-tune smaller models (Macina et al., 2023) and train teachers and teaching assistants through simulating students (Markel et al., 2023; Lee et al., 2023; Yue et al., 2024). In the field of computer science, Kasneci et al. (2023) and Becker et al. (2023) highlighted the potentials and challenges, with Kasneci et al. (2023) advocating for multilingualism in LLM-powered tools. Kazemitabaar et al. (2024) developed an LLM-based coding assistant that provides guidance without providing direct solutions. In conclusion, these developments illustrate the growing role of LLMs in reducing biases, saving time, and providing valuable feedback for learners (Li \& Liu, 2024).



% \subsection{Multilingual LLMs}
% \subsubsection{MLLMs} In comparison to a monolingual large language model (LLM), which can only process one language at a time,  Multilingual Large Language Models (MLLMs) have the ability to process and produce text in multiple languages (L Qin et al., 2024). These models are trained on data from different languages, learning to complete general NLP tasks such as reasoning, summarization, and question answering (Yupeng, et al. 2024). Given the emerging nature of this technology, researchers most often test the reliability of such models with multilingual benchmarks in non-English languages (Ahuja et al. 2024, Team et al. 2022) and human evaluation (Team et al. 2022, Jin \& Chandra 2023). Because these extremely popular models, such as ChatGPT, Llama 3.1, Mistral, and Gemma, are used daily by millions around the world, examining the limitations of MLLMs is crucial for greater accessibility and fairness.

% \subsubsection{Biases in MLLMs} In the conversation of bringing MLLM tools into wide-spread use and classrooms, bias is a major concern. In numerous studies on multilingual evaluation, it is shown that popular MLLMs, ChatGPT, Mistral, Llama 2, BLOOM, and Gemma, consistently perform better on various tasks in English versus non-English languages (Jin \& Chandra 2023, Ahuja et al. 2024, Lai et al. 2024, Bang et al. 2023). When MLLMs such as Llama 3.1 has roughly 5\% multilingual pretraining data (sourced from meta website) and GPT-4 pretraining data is similarly English-centric (OpenAI 2023), MLLM language disparities become apparent. Depending on the availability of data, many language groups are poorly represented in NLP technologies, systematically excluding spoken languages in multilingual communities and languages with few digitized sources (Joshi et al. 2021). With these uneven and English-centric data distributions, MLLM research and benchmark evaluation are catered towards English speakers, lacking the representation needed to support multilingualism. As these NLP technologies expand to support users worldwide, the examination into the fairness of MLLMs is vital; these limitations not only affect their utility in educational contexts but also raises broader issues of social justice.

% \subsubsection{MLLMs Code Switching} With newer and more advanced models, the current generation of MLLMs have significantly improved in their multilingual abilities (Zhu et al. 2024, Ahuja et al 2024). In translation tasks, state-of-the-art MLLMs demonstrate increasing capabilities, most noteworthy is GPT-4 outperforming its predecessor GPT-3.5 and various open-source models (Zhu et al. 2024, Ahuja et al 2024). Additionally, research efforts in accurately evaluating MLLMs for code-switching have yielded two well-known code-switching benchmarks GlueCoS (Khanuja et al. 2020) and LinCE (Aguilar et al. 2020). Though these research efforts reveal a promising direction for MLLM translanguaging capabilities, upon further inspection, there is still lack of support for code-switching ability in many MLLMs (Zhang et al. 2023). 

% Although previous generations of MLLMs fall short in translanguaging capabilities such as code-switching (Yong et al. 2023, Zhang et al. 2023), recent studies have shown that certain newer MLLMs demonstrate robusticity for code-switching and cross-lingual understanding (Huzaifah et al. 2024). Comparing different methods of machine translations, Huzaifah et al. (2024) found that GPT-4 performed the best on seven multilingual translation benchmarks, followed closely by GPT-3.5. These two models in particular handled code-switch inputs more robustly than commercial engines Google Translate and DeepL Translate, with other (open-source) MLLMs (Bard-PALM2, Llama-2-70B, Falcon-40B, and Phoenix-7B) lagging behind in performance. For these open-source models, it is proposed that the lack of code-switching ability stems from the distribution of data used in LLM training. When training data does not include text alternating languages, the homogeneity of data fails to prepare MLLMs for code-switching (Yong et al. 2023). The problem can be attributed to the complexity of acquiring accurate data and annotations from non-English language varieties, resulting in a lack of code-switching resources (1. Zhang et al. 2023). Historically, code-switching was viewed as a predominantly ‘colloquial’ or spoken phenomenon; now with new technology, code-switching is recorded in writing via social-media and voice-operated devices (Winata et al. 2023). However, human annotations and checks are still required for creating high-quality datasets from these texts. In light of these constraints, many NLP researchers have alternatively explored using synthetic code-switched datasets to overcome the data scarcity (Laureano De Leon et al. 2024, Pratapa et al. 2018). Notably, Laureano De Leon et al. 2024 manually create a code-switching dataset using replacements in randomly selected language (within pairs) and noun-phrase translations. Alternatively, Hu et al. (2023) and Yong et al. (2023) explore utilizing MLLMs to generate synthetic code-switching to address the data deficit. Yong et al. (2023) prompt various MLLMs to generate synthetic code-switching texts in South East Asian languages, finding ChatGPT (GPT-3.5) outperforms open-source MLLMs in generating code-switched texts. With access to these synthetic datasets, researchers are able to overcome data scarcities for low-resource languages and code-switching contexts. For instance, Santy et al (2021) uses a synthetic code-switched dataset to finetune open-source MLLM mBERT, improving its code-switching performance. These discoveries have growing implications for the bi-/multilingual community as AI tools are increasingly becoming more common in educational contexts. Since emergent bilingual learners engage in classroom discussions in two or more languages, it is important to develop fair and reliable technology that captures this dynamic process instead of limiting NLP users to monolingual interactions. By employing similar methods to investigate the code-switching abilities of MLLMs, we aim to develop strategies and tools more representative of bi-/multilingual speakers. 




% \rucomment{This section can be used to clarify to the reader a) how different your work is from similar papers and b) how does your work fit into the larger body of the literature. For this, it's a nice idea to categorize all the papers into 2-3 groups, and give each group 1-2 paragraphs.}

% Cite a paper by doing \verb|\cite{Abril07}|. 
% % Command is \cite{bibtex name of article}


==> Sections/ethical_considerations.tex <==
\section{Ethical Considerations}
\label{sec:ethical-considerations}



==> Sections/limitations.tex <==
\section{Limitations}
\label{sec:limitations}



==> references_sorted_occurrence.tex <==
@inproceedings{karumbaiah2021using,
  title={Using past data to warm start active machine learning: Does context matter?},
  author={Karumbaiah, Shamya and Lan, Andrew and Nagpal, Sachit and Baker, Ryan S and Botelho, Anthony and Heffernan, Neil},
  booktitle={LAK21: 11th International Learning Analytics and Knowledge Conference},
  pages={151--160},
  year={2021}
}

@article{shams2023ai,
  title={AI and the quest for diversity and inclusion: A systematic literature review},
  author={Shams, Rifat Ara and Zowghi, Didar and Bano, Muneera},
  journal={AI and Ethics},
  pages={1--28},
  year={2023},
  publisher={Springer}
}

@article{anis2023leveraging,
  title={Leveraging artificial intelligence for inclusive English language teaching: Strategies and implications for learner diversity},
  author={Anis, Muneeba},
  journal={Journal of Multidisciplinary Educational Research},
  volume={12},
  number={6},
  pages={54--70},
  year={2023}
}

@article{bang2023multitask,
  title={A multitask, multilingual, multimodal evaluation of chatgpt on reasoning, hallucination, and interactivity},
  author={Bang, Yejin and Cahyawijaya, Samuel and Lee, Nayeon and Dai, Wenliang and Su, Dan and Wilie, Bryan and Lovenia, Holy and Ji, Ziwei and Yu, Tiezheng and Chung, Willy and others},
  journal={arXiv preprint arXiv:2302.04023},
  year={2023}
}

@article{zhang2023multilingual,
  title={Multilingual large language models are not (yet) code-switchers},
  author={Zhang, Ruochen and Cahyawijaya, Samuel and Cruz, Jan Christian Blaise and Winata, Genta Indra and Aji, Alham Fikri},
  journal={arXiv preprint arXiv:2305.14235},
  year={2023}
}

@article{yong2023prompting,
  title={Prompting multilingual large language models to generate code-mixed texts: The case of south east asian languages},
  author={Yong, Zheng-Xin and Zhang, Ruochen and Forde, Jessica Zosa and Wang, Skyler and Subramonian, Arjun and Lovenia, Holy and Cahyawijaya, Samuel and Winata, Genta Indra and Sutawika, Lintang and Cruz, Jan Christian Blaise and others},
  journal={arXiv preprint arXiv:2303.13592},
  year={2023}
}

@article{qin2024multilingual,
  title={Multilingual large language model: A survey of resources, taxonomy and frontiers},
  author={Qin, Libo and Chen, Qiguang and Zhou, Yuhang and Chen, Zhi and Li, Yinghui and Liao, Lizi and Li, Min and Che, Wanxiang and Yu, Philip S},
  journal={arXiv preprint arXiv:2404.04925},
  year={2024}
}

@article{garcia2017translanguaging,
  title={Translanguaging in bilingual education},
  author={Garc{\'\i}a, Ofelia and Lin, Angel MY and others},
  journal={Bilingual and multilingual education},
  pages={117--130},
  year={2017}
}

@article{hamman2018translanguaging,
  title={Translanguaging and positioning in two-way dual language classrooms: A case for criticality},
  author={Hamman, Laura},
  journal={Language and Education},
  volume={32},
  number={1},
  pages={21--42},
  year={2018},
  publisher={Taylor \& Francis}
}

@article{WEI20111222,
    title = {Moment Analysis and translanguaging space: Discursive construction of identities by multilingual Chinese youth in Britain},
    journal = {Journal of Pragmatics},
    volume = {43},
    number = {5},
    pages = {1222-1235},
    year = {2011},
    note = {Multilingual structures and agencies},
    issn = {0378-2166},
    doi = {https://doi.org/10.1016/j.pragma.2010.07.035},
    url = {https://www.sciencedirect.com/science/article/pii/S0378216610002535},
    author = {Li Wei},
    keywords = {Translanguaging, Social space, Multilingual practices, Youth, Chinese}
}

@article{wei2018translanguaging,
  title={Translanguaging as a practical theory of language},
  author={Wei, Li},
  journal={Applied linguistics},
  volume={39},
  number={1},
  pages={9--30},
  year={2018},
  publisher={Oxford University Press}
}

@article{hesson2014translanguaging,
  title={Translanguaging in curriculum and instruction: A CUNY-NYSIEB guide for educators},
  author={Hesson, Sarah and Seltzer, Kate and Woodley, Heather H},
  journal={New York: CUNY-NYSIEB},
  year={2014}
}

@article{otheguy2015clarifying,
  title={Clarifying translanguaging and deconstructing named languages: A perspective from linguistics},
  author={Otheguy, Ricardo and Garc{\'\i}a, Ofelia and Reid, Wallis},
  journal={Applied linguistics review},
  volume={6},
  number={3},
  pages={281--307},
  year={2015},
  publisher={De Gruyter Mouton}
}

@article{zhu2023multilingual,
  title={Multilingual machine translation with large language models: Empirical results and analysis},
  author={Zhu, Wenhao and Liu, Hongyi and Dong, Qingxiu and Xu, Jingjing and Huang, Shujian and Kong, Lingpeng and Chen, Jiajun and Li, Lei},
  journal={arXiv preprint arXiv:2304.04675},
  year={2023}
}

@article{ahuja2023megaverse,
  title={Megaverse: Benchmarking large language models across languages, modalities, models and tasks},
  author={Ahuja, Sanchit and Aggarwal, Divyanshu and Gumma, Varun and Watts, Ishaan and Sathe, Ashutosh and Ochieng, Millicent and Hada, Rishav and Jain, Prachi and Axmed, Maxamed and Bali, Kalika and others},
  journal={arXiv preprint arXiv:2311.07463},
  year={2023}
}

@article{choudhury2023ask,
  title={Ask Me in English Instead: Cross-Lingual Evaluation of Large Language Models for Healthcare Queries},
  author={Choudhury, De and others},
  journal={arXiv preprint arXiv:2310.13132},
  year={2023}
}

@article{achiam2023gpt,
  title={Gpt-4 technical report},
  author={Achiam, Josh and Adler, Steven and Agarwal, Sandhini and Ahmad, Lama and Akkaya, Ilge and Aleman, Florencia Leoni and Almeida, Diogo and Altenschmidt, Janko and Altman, Sam and Anadkat, Shyamal and others},
  journal={arXiv preprint arXiv:2303.08774},
  year={2023}
}

@article{joshi2020state,
  title={The state and fate of linguistic diversity and inclusion in the NLP world},
  author={Joshi, Pratik and Santy, Sebastin and Budhiraja, Amar and Bali, Kalika and Choudhury, Monojit},
  journal={arXiv preprint arXiv:2004.09095},
  year={2020}
}

@article{winata2022decades,
  title={The decades progress on code-switching research in nlp: A systematic survey on trends and challenges},
  author={Winata, Genta Indra and Aji, Alham Fikri and Yong, Zheng-Xin and Solorio, Thamar},
  journal={arXiv preprint arXiv:2212.09660},
  year={2022}
}

@article{laureano2024code,
  title={Code-Mixed Probes Show How Pre-Trained Models Generalise On Code-Switched Text},
  author={Laureano De Leon, Frances A and Tayyar Madabushi, Harish and Lee, Mark},
  journal={arXiv e-prints},
  pages={arXiv--2403},
  year={2024}
}

@inproceedings{hu2023improving,
  title={Improving multilingual and code-switching asr using large language model generated text},
  author={Hu, Ke and Sainath, Tara N and Li, Bo and Zhang, Yu and Cheng, Yong and Wang, Tao and Zhang, Yujing and Liu, Frederick},
  booktitle={2023 IEEE Automatic Speech Recognition and Understanding Workshop (ASRU)},
  pages={1--7},
  year={2023},
  organization={IEEE}
}

@inproceedings{huzaifah2024evaluating,
  title={Evaluating Code-Switching Translation with Large Language Models},
  author={Huzaifah, Muhammad and Zheng, Weihua and Chanpaisit, Nattapol and Wu, Kui},
  booktitle={Proceedings of the 2024 Joint International Conference on Computational Linguistics, Language Resources and Evaluation (LREC-COLING 2024)},
  pages={6381--6394},
  year={2024}
}

@article{li2023synthetic,
  title={Synthetic data generation with large language models for text classification: Potential and limitations},
  author={Li, Zhuoyan and Zhu, Hangxiao and Lu, Zhuoran and Yin, Ming},
  journal={arXiv preprint arXiv:2310.07849},
  year={2023}
}


@article{hesson2014translanguaging,
  title={Translanguaging in curriculum and instruction: A CUNY-NYSIEB guide for educators},
  author={Hesson, Sarah and Seltzer, Kate and Woodley, Heather H},
  journal={New York: CUNY-NYSIEB},
  year={2014}
}

@article{li2024applying,
  title={Applying large language models for automated essay scoring for non-native Japanese},
  author={Li, Wenchao and Liu, Haitao},
  journal={Humanities and Social Sciences Communications},
  volume={11},
  number={1},
  pages={1--15},
  year={2024},
  publisher={Palgrave}
}

@Article{languages7030220,
AUTHOR = {Nguyen, Li and Yuan, Zheng and Seed, Graham},
TITLE = {Building Educational Technologies for Code-Switching: Current Practices, Difficulties and Future Directions},
JOURNAL = {Languages},
VOLUME = {7},
YEAR = {2022},
NUMBER = {3},
ARTICLE-NUMBER = {220},
URL = {https://www.mdpi.com/2226-471X/7/3/220},
ISSN = {2226-471X},
ABSTRACT = {Code-switching (CSW) is the phenomenon where speakers use two or more languages in a single discourse or utterance—an increasingly recognised natural product of multilingualism in many settings. In language teaching and learning in particular, code-switching has been shown to bring in many pedagogical benefits, including accelerating students’ confidence, increasing their access to content, as well as improving their participation and engagement. Unfortunately, however, current educational technologies are not yet able to keep up with this ‘multilingual turn’ in education, and are partly responsible for the constraint of this practice to only classroom contexts. In an effort to make progress in this area, we offer a data-driven position paper discussing the current state of affairs, difficulties of the existing educational natural language processing (NLP) tools for CSW and possible directions for future work. We specifically focus on two cases of feedback and assessment technologies, demonstrating how the current state-of-the-art in these domains fails with code-switching data due to a lack of appropriate training data, lack of robust evaluation benchmarks and lack of end-to-end user-facing educational applications. We present some empirical user cases of how CSW manifests and suggest possible technological solutions for each of these scenarios.},
DOI = {10.3390/languages7030220}
}

@article{chen2016building,
  title={Building e-rater{\textregistered} scoring models using machine learning methods},
  author={Chen, Jing and Fife, James H and Bejar, Isaac I and Rupp, Andr{\'e} A},
  journal={ETS Research Report Series},
  volume={2016},
  number={1},
  pages={1--12},
  year={2016},
  publisher={Wiley Online Library}
}

@article{chodorow2004beyond,
  title={Beyond essay length: evaluating e-rater{\textregistered}'s performance on toefl{\textregistered} essays},
  author={Chodorow, Martin and Burstein, Jill},
  journal={ETS Research Report Series},
  volume={2004},
  number={1},
  pages={i--38},
  year={2004},
  publisher={Wiley Online Library}
}

@inproceedings{hirao-etal-2020-automated,
    title = "Automated Essay Scoring System for Nonnative {J}apanese Learners",
    author = "Hirao, Reo  and
      Arai, Mio  and
      Shimanaka, Hiroki  and
      Katsumata, Satoru  and
      Komachi, Mamoru",
    editor = "Calzolari, Nicoletta  and
      B{\'e}chet, Fr{\'e}d{\'e}ric  and
      Blache, Philippe  and
      Choukri, Khalid  and
      Cieri, Christopher  and
      Declerck, Thierry  and
      Goggi, Sara  and
      Isahara, Hitoshi  and
      Maegaard, Bente  and
      Mariani, Joseph  and
      Mazo, H{\'e}l{\`e}ne  and
      Moreno, Asuncion  and
      Odijk, Jan  and
      Piperidis, Stelios",
    booktitle = "Proceedings of the Twelfth Language Resources and Evaluation Conference",
    month = may,
    year = "2020",
    address = "Marseille, France",
    publisher = "European Language Resources Association",
    url = "https://aclanthology.org/2020.lrec-1.157",
    pages = "1250--1257",
    abstract = "In this study, we created an automated essay scoring (AES) system for nonnative Japanese learners using an essay dataset with annotations for a holistic score and multiple trait scores, including content, organization, and language scores. In particular, we developed AES systems using two different approaches: a feature-based approach and a neural-network-based approach. In the former approach, we used Japanese-specific linguistic features, including character-type features such as {``}kanji{''} and {``}hiragana.{''} In the latter approach, we used two models: a long short-term memory (LSTM) model (Hochreiter and Schmidhuber, 1997) and a bidirectional encoder representations from transformers (BERT) model (Devlin et al., 2019), which achieved the highest accuracy in various natural language processing tasks in 2018. Overall, the BERT model achieved the best root mean squared error and quadratic weighted kappa scores. In addition, we analyzed the robustness of the outputs of the BERT model. We have released and shared this system to facilitate further research on AES for Japanese as a second language learners.",
    language = "English",
    ISBN = "979-10-95546-34-4",
}

@ARTICLE{10520824,
  author={Song, Yishen and Zhu, Qianta and Wang, Huaibo and Zheng, Qinhua},
  journal={IEEE Transactions on Learning Technologies}, 
  title={Automated Essay Scoring and Revising Based on Open-Source Large Language Models}, 
  year={2024},
  volume={17},
  number={},
  pages={1920-1930},
  keywords={Task analysis;Chatbots;Vocabulary;Engines;Standards;Long short term memory;Electronic mail;Assessment;automated essay revising (AER);automated essay scoring (AES);generative artificial intelligence;open-source large language model (LLM)},
  doi={10.1109/TLT.2024.3396873}}

@article{anderson2021translingual,
  title={Translingual practices in English classrooms in India: Current perceptions and future possibilities},
  author={Anderson, Jason and Lightfoot, Amy},
  journal={International Journal of Bilingual Education and Bilingualism},
  year={2021},
  publisher={Taylor \& Francis}
}

@misc{stahl2024exploringllmpromptingstrategies,
      title={Exploring LLM Prompting Strategies for Joint Essay Scoring and Feedback Generation}, 
      author={Maja Stahl and Leon Biermann and Andreas Nehring and Henning Wachsmuth},
      year={2024},
      eprint={2404.15845},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2404.15845}, 
}

@article{MEYER2024100199,
title = {Using LLMs to bring evidence-based feedback into the classroom: AI-generated feedback increases secondary students’ text revision, motivation, and positive emotions},
journal = {Computers and Education: Artificial Intelligence},
volume = {6},
pages = {100199},
year = {2024},
issn = {2666-920X},
doi = {https://doi.org/10.1016/j.caeai.2023.100199},
url = {https://www.sciencedirect.com/science/article/pii/S2666920X23000784},
author = {Jennifer Meyer and Thorben Jansen and Ronja Schiller and Lucas W. Liebenow and Marlene Steinbach and Andrea Horbach and Johanna Fleckenstein},
keywords = {Secondary education, Improving classroom teaching, Applications in subject areas},
abstract = {Writing proficiency is an essential skill for upper secondary students that can be enhanced through effective feedback. Creating feedback on writing tasks, however, is time-intensive and presents a challenge for educators, often resulting in students receiving insufficient or no feedback. The advent of text-generating large language models (LLMs) offers a promising solution, namely, automated evidence-based feedback generation. Yet, empirical evidence from randomized controlled studies about the effectiveness of LLM-generated feedback is missing. To address this issue, the current study compared the effectiveness of LLM-generated feedback to no feedback. A sample of N = 459 upper secondary students of English as a foreign language wrote an argumentative essay. Students in the experimental group were asked to revise their text according to feedback that was generated using the LLM GPT-3.5-turbo. The control group revised their essays without receiving feedback. We assessed improvement in the revision using automated essay scoring. The results showed that LLM-generated feedback increased revision performance (d = .19) and task motivation (d = 0.36). Moreover, it increased positive emotions (d = 0.34) compared to revising without feedback. The findings highlight that using LLMs allows to create timely feedback that can positively relate to students’ cognitive and affective-motivational outcomes. Future perspectives and the implications for research and practice of using LLM-generated feedback in intelligent tutoring systems are discussed.}
}

@misc{mcnichols2023automated,
  title={Automated distractor and feedback generation for math multiple-choice questions via in-context learning},
  author={McNichols, Hunter and Feng, Wanyong and Lee, Jaewook and Scarlatos, Alexander and Smith, Digory and Woodhead, Simon and Lan, Andrew},
  year={2023},
  publisher={NeurIPS}
}

@article{bulusuautomated,
  title={An Automated Graphing System for Mathematical Pedagogy},
  author={Bulusu, Arya and Man, Brandon and Jagmohan, Ashish and Vempaty, Aditya and Mari-Wyka, Jennifer}
}

@article{Markel2023GPTeachIT,
  title={GPTeach: Interactive TA Training with GPT-based Students},
  author={Julia M. Markel and Steven G. Opferman and James A. Landay and Chris Piech},
  journal={Proceedings of the Tenth ACM Conference on Learning @ Scale},
  year={2023},
  url={https://api.semanticscholar.org/CorpusID:259949836}
}

@inproceedings{LeeGenerativeAF,
  title={Generative Agent for Teacher Training: Designing Educational Problem-Solving Simulations with Large Language Model-based Agents for Pre-Service Teachers},
  author={Unggi Lee and Sanghyeok Lee and Junbo Koh and Yeil Jeong and Haewon Jung and Gyuri Byun and Jewoong Moon and Jieun Lim and † HyeoncheolKim},
  url={https://api.semanticscholar.org/CorpusID:266874743}
}

@article{meta_llama3_2024,
    title = {Introducing Meta Llama 3: The most capable openly available LLM to date},
    author = {Meta AI},
    year = {2024},
    url = {https://ai.meta.com/llama/}
}

